L2 Orthogonal Space Time Code for Continuous Phase Modulation

To combine the high power efficiency of Continuous Phase Modulation (CPM) with either high spectral efficiency or enhanced performance in low Signal to Noise conditions, some authors have proposed to introduce CPM in a MIMO frame, by using Space Time Codes (STC). In this paper, we address the code design problem of Space Time Block Codes combined with CPM and introduce a new design criterion based on L2 orthogonality. This L2 orthogonality condition, with the help of simplifying assumption, leads, in the 2x2 case, to a new family of codes. These codes generalize the Wang and Xia code, which was based on pointwise orthogonality. Simulations indicate that the new codes achieve full diversity and a slightly better coding gain. Moreover, one of the codes can be interpreted as two antennas fed by two conventional CPMs using the same data but with different alphabet sets. Inspection of these alphabet sets lead also to a simple explanation of the (small) spectrum broadening of Space Time Coded CPM.

==> picture1.tex <==
% Generated with LaTeXDraw 1.9.3
% Mon Jan 14 22:08:57 GMT 2008
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\scalebox{0.93} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-1.4928125)(9.028438,1.4728125)
\psframe[linewidth=0.04,dimen=outer](1.269375,0.8528125)(0.669375,-0.9471875)
\psframe[linewidth=0.04,dimen=outer](2.769375,0.9528125)(1.969375,-0.9471875)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(0.169375,-0.0471875)(0.669375,-0.0471875)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.269375,0.4528125)(1.969375,0.4528125)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(1.269375,-0.5471875)(1.969375,-0.5471875)
\psline[linewidth=0.04cm](2.769375,0.4528125)(3.769375,0.4528125)
\psline[linewidth=0.04cm](2.769375,-0.5471875)(3.769375,-0.5471875)
\usefont{T1}{ptm}{m}{n}
\rput{90.0}(1.5001563,-1.5164063){\rput(1.4904687,0.4628125){Mapping}}
\usefont{T1}{ptm}{m}{n}
\rput(0.43359375,0.2628125){$d_j$}
\usefont{T1}{ptm}{m}{n}
\rput(1.5635937,0.7628125){$d_{1r}^{(i)}$}
\usefont{T1}{ptm}{m}{n}
\rput(1.5635937,-0.2371875){$d_{2r}^{(i)}$}
\usefont{T1}{ptm}{m}{n}
\rput{90.0}(2.8326561,-2.8657813){\rput(2.8314064,0.4628125){Modulation}}
\psline[linewidth=0.04cm](3.769375,-0.0471875)(3.769375,-0.5471875)
\psline[linewidth=0.04cm](3.569375,-0.0471875)(3.769375,-0.3471875)
\psline[linewidth=0.04cm](3.769375,-0.3471875)(3.969375,-0.0471875)
\psline[linewidth=0.04cm](3.769375,0.9528125)(3.769375,0.4528125)
\psline[linewidth=0.04cm](3.569375,0.9528125)(3.769375,0.6528125)
\psline[linewidth=0.04cm](3.769375,0.6528125)(3.969375,0.9528125)
\usefont{T1}{ptm}{m}{n}
\rput(3.1835938,0.6628125){$s_{1r}(t)$}
\usefont{T1}{ptm}{m}{n}
\rput(3.1835938,-0.3371875){$s_{2r}(t)$}
\psline[linewidth=0.04cm](4.569375,1.4528126)(4.569375,0.9528125)
\psline[linewidth=0.04cm](4.369375,1.4528126)(4.569375,1.1528125)
\psline[linewidth=0.04cm](4.569375,1.1528125)(4.769375,1.4528126)
\psline[linewidth=0.04cm](4.569375,0.4528125)(4.569375,-0.0471875)
\psline[linewidth=0.04cm](4.369375,0.4528125)(4.569375,0.1528125)
\psline[linewidth=0.04cm](4.569375,0.1528125)(4.769375,0.4528125)
\psline[linewidth=0.04cm](4.569375,-0.5471875)(4.569375,-1.0471874)
\psline[linewidth=0.04cm](4.369375,-0.5471875)(4.569375,-0.8471875)
\psline[linewidth=0.04cm](4.569375,-0.8471875)(4.769375,-0.5471875)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.569375,0.9528125)(5.669375,0.9528125)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.569375,-0.0471875)(5.669375,-0.0471875)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(4.569375,-1.0471874)(5.669375,-1.0471874)
\usefont{T1}{ptm}{m}{n}
\rput{-90.0}(3.7592187,5.1342187){\rput(4.4126563,0.8628125){...}}
\usefont{T1}{ptm}{m}{n}
\rput{-90.0}(4.7592187,4.1342187){\rput(4.4126563,-0.1371875){...}}
\psframe[linewidth=0.04,dimen=outer](6.469375,1.1528125)(5.669375,-1.2471875)
\psframe[linewidth=0.04,dimen=outer](7.869375,1.1528125)(7.169375,-1.2471875)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.469375,0.7528125)(7.169375,0.7528125)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(6.469375,-0.9471875)(7.169375,-0.9471875)
\psline[linewidth=0.04cm,arrowsize=0.05291667cm 2.0,arrowlength=1.4,arrowinset=0.4]{->}(7.869375,-0.0471875)(8.369375,-0.0471875)
\usefont{T1}{ptm}{m}{n}
\rput{90.0}(7.032656,-7.320781){\rput(7.1426563,0.2628125){...dist...}}
\usefont{T1}{ptm}{m}{n}
\rput{90.0}(7.8771877,-8.173437){\rput(8.0075,0.3628125){MLSE}}
\usefont{T1}{ptm}{m}{n}
\rput{90.0}(6.51125,-6.549375){\rput(6.5103126,0.4628125){Detection}}
\usefont{T1}{ptm}{m}{n}
\rput(8.063594,0.2628125){$\hat d_j$}
\usefont{T1}{ptm}{m}{n}
\rput(5.103594,1.2628125){$y_{1}(t)$}
\usefont{T1}{ptm}{m}{n}
\rput(5.0935936,0.2628125){$y_n(t)$}
\usefont{T1}{ptm}{m}{n}
\rput(5.193594,-0.7371875){$y_{L_r}(t)$}
\end{pspicture} 
}


